Task-Adaptive Pseudo Labeling for Transductive Meta-Learning

Meta-learning performs adaptation through a limited amount of support set, which may cause a sample bias problem. To solve this problem, transductive meta-learning is getting more and more attention, going beyond the conventional inductive learning perspective. This paper proposes so-called task-adaptive pseudo labeling for transductive meta-learning. Specifically, pseudo labels for unlabeled query sets are generated from labeled support sets through label propagation. Pseudo labels enable to adopt the supervised setting as it is and also use the unlabeled query set in the adaptation process. As a result, the proposed method is able to deal with more examples in the adaptation process than inductive ones, which can result in better classification performance of the model. Note that the proposed method is the first approach of applying task adaptation to pseudo labeling. Experiments show that the proposed method outperforms the state-of-the-art (SOTA) technique in 5-way 1-shot few-shot classification.

==> Article Title/materials/algorithm.tex <==
\begin{algorithm}[t]\small
% \fontsize{9}{11}\selectfont
\caption{Task-Adaptive Pseudo Labeling (TAPL)}

% https://tex.stackexchange.com/questions/200186/how-to-wrap-lines-correctly-inside-algorithmic
\makeatletter
\newcommand{\algmargin}{\the\ALG@thistlm}
\makeatother
\algnewcommand{\parState}[1]{\State%
  \parbox[t]{\dimexpr\linewidth-\algmargin}{\strut #1\strut}}

\textbf{Require: } $\beta, \eta$: Learning rates\\
\textbf{Require: } $J$: The number of inner-loop update steps

\begin{algorithmic}[1]
\State Randomly initialize $\boldtheta$, $\boldphi$, and $\boldpsi$

\While{not done}
    %\State sample mini-batch of tasks $\task \sim p(\mathcal{T})$
    \State Sample $B$ numbers of mini-batch of the current task
    
    \For{$i \in [B]$}
        \State $\boldtheta_{i} \gets \boldtheta$
        \State $\boldphi_{i} \gets \boldphi$
        \State $\dataset = \{ \support, \query \}$
        
        % \parState {%
        %         \textcolor{\red}{\textit{// Inner loop}}
        %         }
        \For {$j \in [J]$ }
            \State Compute $\pi_{\boldtheta_{i}}(\dataset)$
            % \parState {%
            %     \textcolor{ForestGreen}{\textit{// Task-adaptation}}
            %     }
            \parState {%
                Get task representation $\boldtau_{i,j}$}
            \parState {%
                Generate task-adaptation parameters for $g_{\boldphi_{i}}$:\\
                $\{ \gamma^{\ell}_{i} \}_{\ell=1}^{L} = h_{\boldpsi}(\boldtau_{i,j})$}
            \parState {%
                Make the parameters $\boldphi_{i}$ adapted on the current task:\\
                $\{ \boldphi^{\ell}_{i} \}_{\ell=1}^{L} \gets \{ \gamma^{\ell}_{i} \boldphi^{\ell}_{i} \}_{\ell=1}^{L}$}
            % \parState {%
            %     \textcolor{ForestGreen}{\textit{// Label propagation}}
            %     }
            \parState {%
                Generate pseudo labels for the unlabeled query sets:\\
                $\hat{y}_{\query}=\argmax{g_{\boldphi_{i}}(\pi_{\boldtheta_{i}}(\dataset))}$}
            \State Concatenate the labels: $y_{\dataset} = \{ y_{\support}, \hat{y}_{\query} \}$
            \parState {%
                Compute inner loop loss: $\mathcal{L}(\pi_{\boldtheta_{i}}(\dataset), y_{\dataset})$}
            \parState {%
                Perform gradient descent:\\
                $\boldtheta_{i} \gets \boldtheta_{i} - \beta \nabla_{\boldtheta_{i}} \mathcal{L}(\pi_{\boldtheta_{i}}(\dataset), y_{\dataset})$}
        \EndFor
    % \parState {%
    %     \textcolor{Orange}{\textit{// Outer loop}}
    %     }
    \parState{% 
        Compute outer loop loss:\\
        $\mathcal{L}_{i} = \dfrac{1}{2}(\mathcal{L}(\pi_{\boldtheta_{i}}(\query), y_{\query}) + 
        \mathcal{L}(g_{\boldphi_{i}}(\pi_{\boldtheta_{i}}(\mathcal{D}_{i})), y_{\query}))$}
    \EndFor
    
    % \State $(\boldtheta, \boldphi) \gets (\boldtheta, \boldphi) - \eta \nabla_{(\boldtheta, \boldphi)}\sum_{i=1}^{B} \mathcal{L}(\boldtheta_{i};\query)$
    \parState {%
        Update the model parameters: \\
        % $(\boldtheta, \boldphi, \boldpsi, \alpha) \gets (\boldtheta, \boldphi, \boldpsi, \alpha) - \eta \nabla_{(\boldtheta, \boldphi, \boldpsi, \alpha)}\sum_{i=1}^{B} \mathcal{L}_{i}$
        $(\boldtheta, \boldphi, \boldpsi) \gets (\boldtheta, \boldphi, \boldpsi) - \eta \nabla_{(\boldtheta, \boldphi, \boldpsi)}\sum_{i=1}^{B} \mathcal{L}_{i}$
        }
    
\EndWhile

\end{algorithmic}
\label{alg:TAPL}
\end{algorithm}

==> Article Title/materials/fig1.tex <==
% \begin{figure}
% \begin{center}
%     \centering
%         \subfloat[]{\includegraphics[width=0.45\linewidth]{materials/images/inductive.png}}
%         % \caption{Inductive learning}
%     % \end{subfigure}
%     % \hspace{3mm}
%     \hfil
%     % \begin{subfigure}{.45\linewidth}
%         \subfloat[]{\includegraphics[width=0.45\linewidth]{materials/images/transductive.png}}
%         % \caption{Transductive learning}
%     % \setlength{\abovecaptionskip}{2pt}
%     % \setlength{\belowcaptionskip}{10pt}
% \end{center}
%     \setlength{\abovecaptionskip}{10pt}
%     % \setlength{\belowcaptionskip}{-5pt}
%     \caption{Comparison of the (a) inductive and (b) transductive meta-learning. Transductive meta-learning utilizes an unlabeled query set (without edge color) in adaptation, while inductive meta-learning doesn't. Due to the limited number of samples in the support set, inductive meta-learning is vulnerable to suffering sample bias during adaptation.}
% \label{fig1:concept}
% \end{figure}

\begin{figure}[t]
    \begin{center}
        \includegraphics[width=.8\linewidth]{materials/images/inductive_transductive.png}
    \end{center}
    \caption{Comparison of the (a) inductive and (b) transductive meta-learning. Transductive meta-learning utilizes an unlabeled query set (without edge color) in adaptation, while inductive meta-learning doesn't. Due to the limited number of samples in the support set, inductive meta-learning is vulnerable to suffering sample bias during adaptation.}
\label{fig1:concept}
\end{figure}

==> Article Title/materials/fig2.tex <==
\begin{figure*}[t]
    \begin{center}
        \includegraphics[width=\linewidth]{materials/images/TAPL.png}
    \end{center}
    \caption{
    Overview of the proposed method. We generate pseudo labels via label propagation for the unlabeled query set from the support set. 
    Here, a square and a circle denote the examples of the support set and the query set, respectively.
    Each color indicates a class of the current task.
}
\label{fig2:overall}
\end{figure*}

==> Article Title/materials/fig3.tex <==
\begin{figure}[t]
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{5pt}
\begin{center}
    \includegraphics[width=.8\linewidth]{materials/images/embeddings.png}
\end{center}
\caption{Visualization of how pseudo labels are given to the unlabeled query sets in embedding space. Many unlabeled query set samples are given the same label as their ground truth one. Furthermore, the samples with the same pseudo label are embedded closely to each other.}
\label{fig3:visualization}
\end{figure}

==> Article Title/materials/table1_benchmark.tex <==
\begin{table*}[t]
% \setlength{\abovecaptionskip}{0pt}
\caption{Test accuracy of 5-way few-shot classification in miniImageNet and tieredImageNet. Here, `Trans.' indicates the tranductive learning}
%\setlength{\belowcaptionskip}{-5pt}
\begin{center}
\fontsize{6}{6}\selectfont
%\begin{tabular}{c|c|c|c|c}
% \begin{tabularx}{\textwidth}{>{\centering\arraybackslash}X>{\centering\arraybackslash}X
\begin{tabularx}{\textwidth}{>{\arraybackslash}X
>{\centering\arraybackslash}>{\hsize=.3\hsize}X
>{\centering\arraybackslash}>{\hsize=.7\hsize}X
>{\centering\arraybackslash}>{\hsize=.7\hsize}X
>{\centering\arraybackslash}>{\hsize=.7\hsize}X
>{\centering\arraybackslash}>{\hsize=.7\hsize}X}
\toprule %\toprule
\multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{Trans.}} & 
\multicolumn{2}{c}{\textbf{miniImageNet}} & 
\multicolumn{2}{c}{\textbf{tieredImageNet}} \\
%\cmidrule{2-3} %\cmidrule{4-5}
& & \textbf{1-shot} & \textbf{5-shot} & \textbf{1-shot} & \textbf{5-shot} \\
%\tstrut & 1-shot & 5-shot & 1-shot & 5-shot \bstrut \\
\midrule
% MatchingNet~\cite{MatchingNet}  &            &  $43.44 \pm 0.77\%$    & $55.31 \pm 0.73\%$     & --                  & --\\
% RelationNet~\cite{RelationNet}  &            &  $50.44 \pm 0.82\%$    & $65.32 \pm 0.70\%$     & --                  & --\\
% ProtoNet~\cite{ProtoNet}        &            &  $49.42 \pm 0.78\%$    & $68.20 \pm 0.66\%$     & --                  & --\\
% \hdashline
MAML~\cite{MAML}                &            &  $48.70 \pm 1.84\%$    & $63.11 \pm 0.92\%$     & $49.06 \pm 0.50\%$  & $67.48 \pm 0.47\%$\\
% CAVIA (512)~\cite{CAVIA}        &            &  $51.82 \pm 0.65\%$    & $65.85 \pm 0.55\%$     & --                  & --\\
BOIL~\cite{BOIL}                &            &  $49.61 \pm 0.16\%$    & $66.45 \pm 0.37\%$     & $48.58 \pm 0.27\%$  & $69.37 \pm 0.12\%$\\
MAML++~\cite{MAML++}            &            &  $52.15 \pm 0.26\%$    & $68.32 \pm 0.44\%$     & --                  & --\\
ALFA~\cite{ALFA}                &            &  $50.58 \pm 0.51\%$    & $69.12 \pm 0.47\%$     & $53.16 \pm 0.49\%$  & $70.54 \pm 0.46\%$\\
% ModGrad~\cite{ModGrad}          &            &  $53.20 \pm 0.86\%$    & $69.17 \pm 0.69\%$     & --                  & --\\
L2F~\cite{L2F}                  &            &  $52.10 \pm 0.50\%$    & $69.38 \pm 0.46\%$     & $54.40 \pm 0.50\%$  & $73.34 \pm 0.44\%$\\
CxGrad~\cite{CxGrad}            &            & $51.80 \pm 0.46\%$    & $69.82 \pm 0.42\%$      & $55.55 \pm 0.46\%$  & $73.55 \pm 0.41\%$\\
\hdashline
TPN~\cite{TPN}                  & \checkmark & $53.75 \pm 0.86\%$    & $69.43 \pm 0.67\%$      & $57.53 \pm 0.96\%$  & $72.85 \pm 0.74\%$\\
TPN (Higher Shot)~\cite{TPN}    & \checkmark & $55.51 \pm 0.86\%$    & $69.86 \pm 0.65\%$      & $59.91 \pm 0.94\%$  & $73.30 \pm 0.75\%$\\
% MPM~\cite{MPM}                  & \checkmark & 57.59 \%              & 74.02 \%                & 59.44 \%            & \vcsb{76.59\%}\\
MAML++ + SCA~\cite{SCA}         & \checkmark & $54.24 \pm 0.99\%$    & $71.85 \pm 0.53\%$      & --    & --\\
MAML + MeTAL~\cite{MeTAL}       & \checkmark & $52.63 \pm 0.37\%$    & $70.52 \pm 0.29\%$      & $54.34 \pm 0.31\%$  & $70.40 \pm 0.21\%$\\
ALFA + MeTAL~\cite{MeTAL}       & \checkmark & $57.75 \pm 0.38\%$    & \vcsb{74.10 \pm 0.43\%} & $60.29 \pm 0.37\%$  & $75.88 \pm 0.29\%$\\
CxGrad + TAPL (Ours)            & \checkmark & \vcsb{58.55 \pm 0.46\%} & $72.28\pm0.41\%$    & \vcsb{60.58 \pm 0.45\%}    & $75.76 \pm 0.40\%$\\
% \hline
% MAML            & ResNet12 & 51.03 $\pm$ 0.50\% & 68.26 $\pm$ 0.47\% \\
% BOIL            & ResNet12 & -                & 70.50 $\pm$ 0.28\% \\
% L2F             & ResNet12 & 57.48 $\pm$ 0.49\% & 74.68 $\pm$ 0.43\% \\
% CxGrad (Ours)   & - & - \\
\bottomrule
%\end{tabular}
\end{tabularx}
\end{center}
\label{table1:benchmark}
\end{table*}

==> Article Title/materials/table2_ablation.tex <==
\begin{table}[t]
\caption{Ablation study in task-adaptiveness and learnability of $\alpha$ in label propagation.}
%\fontsize{7}{10}\selectfont
\begin{center}
\begin{tabular}{cccc}
\toprule
\textbf{Task-Adaptive} & \textbf{Learnable $\alpha$} & \textbf{iteration time} & \textbf{Accuracy}\\
\midrule
           & \checkmark & 0.709s & $71.22 \pm 0.42\%$ \\
\checkmark & \checkmark & 0.719s & \vcsb{72.28 \pm 0.41\%} \\
\bottomrule
\end{tabular}
\end{center}
\label{table:ablation}
\end{table}

==> Article Title/sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}



==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


